Multi-Stage CNN-Based Monocular 3D Vehicle Localization and Orientation Estimation

This paper aims to design a 3D object detection model from 2D images taken by monocular cameras by combining the estimated bird's-eye view elevation map and the deep representation of object features. The proposed model has a pre-trained ResNet-50 network as its backend network and three more branches. The model first builds a bird's-eye view elevation map to estimate the depth of the object in the scene and by using that estimates the object's 3D bounding boxes. We have trained and evaluate it on two major datasets: a syntactic dataset and the KIITI dataset.

==> dataset_images.tex <==
% \documentclass{article}
% \usepackage{graphicx}
% \usepackage{subcaption}

% \begin{document}

\begin{figure}[h]
\centering
\begin{subfigure}[b]{.49\linewidth}
\includegraphics[width=\linewidth]{images/dataset_sample/SAV_4130_f.png}
\end{subfigure}

\begin{subfigure}[b]{.49\linewidth}
\includegraphics[width=\linewidth]{images/dataset_sample/SAV_44559_f.png}
\end{subfigure}

\begin{subfigure}[b]{.49\linewidth}
\includegraphics[width=\linewidth]{images/dataset_sample/SAV_4130_t.png}
\end{subfigure}

\begin{subfigure}[b]{.49\linewidth}
\includegraphics[width=\linewidth]{images/dataset_sample/SAV_44559_t.png}
\end{subfigure}

\caption{Sample images of the SAV dataset. Top images show the front-view, and bottom images are corresponding to their bird's-eye view~\cite{Palazzi}.}
\label{fig:SAV_Datase}
\end{figure}

% \end{document}

==> layers/init.tex <==
%\ProvidesPackage{init}
\usetikzlibrary{quotes,arrows.meta}
\usetikzlibrary{positioning}

\def\edgecolor{rgb:blue,4;red,1;green,4;black,3}
\newcommand{\midarrow}{\tikz \draw[-Stealth,line width =0.5mm,draw=\edgecolor] (-0.3,0) -- ++(0.3,0);}

\usepackage{Ball}
\usepackage{Box}
\usepackage{RightBandedBox}


